Learning Representations For Images With Hierarchical Labels

Image classification has been studied extensively but there has been limited work in the direction of using non-conventional, external guidance other than traditional image-label pairs to train such models. In this thesis we present a set of methods to leverage information about the semantic hierarchy induced by class labels. In the first part of the thesis, we inject label-hierarchy knowledge to an arbitrary classifier and empirically show that availability of such external semantic information in conjunction with the visual semantics from images boosts overall performance. Taking a step further in this direction, we model more explicitly the label-label and label-image interactions by using order-preserving embedding-based models, prevalent in natural language, and tailor them to the domain of computer vision to perform image classification. Although, contrasting in nature, both the CNN-classifiers injected with hierarchical information, and the embedding-based models outperform a hierarchy-agnostic model on the newly presented, real-world ETH Entomological Collection image dataset https://www.research-collection.ethz.ch/handle/20.500.11850/365379.

==> sections/3/3-algorithm-preliminaries.tex <==
\chapter{Preliminaries}
\label{ch:prelims}
 




==> sections/A/todo.tex <==
\chapter{Running experiments}

\begin{adjustbox}{angle=90}
\begin{tabular}{| c || c | c | c | c | c || c | c || c |} 
 \hline
  Name & Loss & N-dim & im features & batch-size & em lr, im lr & m-F1 & full-F1 & comments  \\ [0.5ex]
 \hline\hline
 ec\_100d\_2xlr\_feat4 & EC & 100 & FC 4 layer & 10*(1+, 10-) & 1e-3, 1e-4 & \textbf{0.7595} & 0.3228 & 600/1000 ep  \\
 ec\_2d\_2xlr\_feat4 & EC & 2 & FC 4 layer & 10*(1+, 10-) & 1e-3, 1e-4 & \underline{0.6068} & 0.1316 & 570/1000 ep \\
 oe\_100d\_2xlr\_feat4 & OE & 100 & FC 4 layer & 10*(1+, 10-) & 1e-3, 1e-4 & 0.1953 & \textbf{0.4498} & 240/1000 ep  \\
 50-50\_hide\_levels/ec\_2d\_2xlr\_init\_5k & EC & 2 & FC 4 layer & 10*(1+, 10-) & 1e-3, 1e-4 & 0.4176 & 0.0736 & 50\% (l, l)+50\% (l, i); level-by-level  \\
 50-50/r18/ec\_2d\_2xlr\_init\_* & EC & 2 & ResNet-18 & 10*(1+, 10-) & 1e-3, 1e-4 & 0.04 & 0.2948 & 50\% (l, l)+50\% (l, i); OVERFITTING!  \\
 50-50/ec\_100d\_2xlr\_init\_5k\_bs100 & EC & 100 & FC 4 layer & 100*(1+, 10-) & 1e-3, 1e-4 & 0.5245 & \underline{0.4185} & 50-50; PROMISING :D 50/1000 ep!  \\
 50-50/ec\_100d\_2xlr\_1e-3im\_init\_5k\_bs100 & EC & 100 & FC 4 layer & 100*(1+, 10-) & 1e-3, 1e-3 & 0.5326 & 0.4164 & 50-50; PROMISING :D 50/1000 ep! \\
 [1ex] \hline
\end{tabular}
\end{adjustbox}

\chapter{To Dos}

\section{11 April, 2019}
\begin{itemize}
  \item Read paper: Hyperbolic Image Embeddings \\
  (https://arxiv.org/pdf/1904.02239.pdf)
  \item log-scale vs dataset frequency; how many have less than 10 samples? 3 samples?
  \item make tables more descriptive and easily readable
  \item check how many outputs are there for the multi-label case? Is it outputing 1s for a lot of labels?
  \item is one threshold always better?
  \item for the d3.js viz; add performance metrics; additionally a heatmap where the nodes are colored based on the performance
  \item is having a weighted sampler helpful? how big of a difference does it make? can we re-weight the loss instead?
  \item Write formal descriptions of each model, loss, hyperparameters, training and eval details, data format, splitting, metrics.
  \item Look at alternative datasets or create one using AMT?
  \item Instead of averaging, we could learn weights for weighted averaging (for multi-level loss)
\end{itemize}
\subsection{Done}
\begin{itemize}
    \item whenever the plot has val, should also have test number for comparison; they should have a very similar trend
    \item Have evaluation metrics per level
    \item add number of train, val, test samples in eval file
    \item include genus level in the ETHEC Merged dataset
    \item Make a histogram that shows number of training samples vs performance
    \item Code profiling
    \item remove classes that have no samples
\end{itemize}

\section{24 April, 2019}
\subsection{Done}
\begin{itemize}
    \item remove classes that have no samples
    \item replace resampling with reweighting the loss
\end{itemize}


\section{3 May, 2019}
\begin{itemize}
  \item use weights per level (2nd baseline)
  \item use more data for testing (shift data from training set); not sure if we want to do this
  \item push the baseline (use more sophisticated CNN backbones)
  \item look at COCO, visual genome, word net and see if some hierarchical dataset can be extracted
  \item next step would be to implement order-embeddings, read the paper again
  \item ask Michael if he would be willing to make the data public
\end{itemize}
\subsection{Done}
\begin{itemize}
    \item write down loss for the two versions for the 3rd baseline
    \item use Adam optimizer
    \item implement constrained version of the 2nd baseline (version 1)
    \item implement constrained version of the 2nd baseline (version 2)
    \item train on black and white images to see the role of color of the butterflies
\end{itemize}

\section{10 May, 2019}
\begin{itemize}
  \item CIFAR100 comes with 2 level hierarchy (check this)
  \item see what the model is focusing on during classification
\end{itemize}
\subsection{Done}
\begin{itemize}
    \item https://paperswithcode.com/task/fine-grained-image-classification
  \item read + summarize papers from Dario and summarize dataset from papers with code
\end{itemize}

\section{16 May, 2019}
\begin{itemize}
  \item -
  
\end{itemize}
\subsection{Done}
\begin{itemize}
    \item Get hierarchical softmax from Dario
    \item what happens when I have loss for different levels
    \item stock and cisse, eccv' 18 paper for visualizing top features (implemented LIME)
\end{itemize}
